Self-Supervised Tracking via Target-Aware Data Synthesis

While deep-learning based tracking methods have achieved substantial progress, they entail large-scale and high-quality annotated data for sufficient training. To eliminate expensive and exhaustive annotation, we study self-supervised learning for visual tracking. In this work, we develop the Crop-Transform-Paste operation, which is able to synthesize sufficient training data by simulating various appearance variations during tracking, including appearance variations of objects and background interference. Since the target state is known in all synthesized data, existing deep trackers can be trained in routine ways using the synthesized data without human annotation. The proposed target-aware data-synthesis method adapts existing tracking approaches within a self-supervised learning framework without algorithmic changes. Thus, the proposed self-supervised learning mechanism can be seamlessly integrated into existing tracking frameworks to perform training. Extensive experiments show that our method 1) achieves favorable performance against supervised learning schemes under the cases with limited annotations; 2) helps deal with various tracking challenges such as object deformation, occlusion, or background clutter due to its manipulability; 3) performs favorably against state-of-the-art unsupervised tracking methods; 4) boosts the performance of various state-of-the-art supervised learning frameworks, including SiamRPN++, DiMP, and TransT.

==> tables/sota_comparison.tex <==
% \begin{table*}[!tb]
% \small
% \renewcommand\arraystretch{1.1} %1.1
%     \caption{\textbf{Experimental results on the OTB100, UAV123, NFS, TrackingNet and LaSOT datasets.} AUC and NPre. denote for the area under the success plot and the normalized precision score. Taking Su-RPN++ which is trained by ourself using the released code as the baseline, the scores in the parentheses show the absolute differences against the baseline. }
%     \label{tab:rs-collect}
%     \centering
% \resizebox{0.98\linewidth}{!}{
%     \begin{tabular}{lccccccc}
%     \toprule
%  \multicolumn{1}{r}{Dataset}   &OTB100 &UAV123 &NFS &\multicolumn{2}{c}{TrackingNet (511 sequences)}&\multicolumn{2}{c}{LaSOT (280 sequences)}\\
%     Tracker    & AUC $\uparrow$& AUC $\uparrow$ & AUC $\uparrow$&  AUC $\uparrow$& NPre. $\uparrow$ &  AUC $\uparrow$&NPre. $\uparrow$ \\
%     \midrule
% SS-RPN++ &\multicolumn{1}{r}{(-1.2) 0.653}   &\multicolumn{1}{r}{(-4.0) 0.552 } &\multicolumn{1}{r}{ (-2.3) 0.464}&65.6 & 73.4&\multicolumn{1}{r}{0.455}&\multicolumn{1}{r}{0.542}\\ 
% Su-RPN++ &\multicolumn{1}{r}{0.665} &\multicolumn{1}{r}{0.592} &\multicolumn{1}{r}{0.487} &\multicolumn{1}{r}{0.677} & \multicolumn{1}{r}{0.764 }&\multicolumn{1}{r}{0.466}&\multicolumn{1}{r}{0.560} \\ 
% SS-Su-RPN++ &\multicolumn{1}{r}{(+2.0) 0.685} &\multicolumn{1}{r}{(+1.4) 0.606} &\multicolumn{1}{r}{(+4.3) 0.530 } &\multicolumn{1}{r}{(+1.4) 0.691} &\multicolumn{1}{r}{(+1.0) 0.774 } &\multicolumn{1}{r}{(+3.3) 0.499 }&\multicolumn{1}{r}{(+3.6) 0.596} \\
% RPN++ (reported)&0.696 &0.613 &- &0.733&0.800 &0.495&0.569\\
%     \bottomrule
%     \end{tabular}}
% \end{table*}

% previous table with precision scores
\begin{table*}[!tb]
\footnotesize
\renewcommand\arraystretch{1.1} %1.1
    \caption{\textbf{Comparisons against other unsupervised and weakly supervised methods on five diverse datasets.}}
    \label{tab:rs-collect}
    \centering
\resizebox{0.98\linewidth}{!}{
    \begin{tabular}{l|rlrlrlrclrcl}
    \toprule
 \multicolumn{1}{r|}{Dataset}   &\multicolumn{2}{c}{OTB100 }&\multicolumn{2}{c}{UAV123 }&\multicolumn{2}{c}{NFS }&\multicolumn{3}{c}{TrackingNet (511 sequences)}&\multicolumn{3}{c}{LaSOT (280 sequences)}\\
    Tracker  & Pre. $\uparrow$ & AUC $\uparrow$& Pre. $\uparrow$& AUC $\uparrow$ & Pre. $\uparrow$& AUC $\uparrow$& Pre. $\uparrow$& AUC $\uparrow$& NPre. $\uparrow$ &  Pre. $\uparrow$& AUC $\uparrow$&NPre. $\uparrow$ \\
    \midrule
UDT~\cite{UDT} &0.781&0.598 &0.696 &0.489&0.406 &0.353&0.479&0.542&0.608 & 0.242&0.265&0.274\\ 
SS-RPN++ (vid)     &0.858&0.634 & 0.774 &0.557 &0.523&0.454&0.588&0.628&0.716&0.432 &0.440&0.529\\ 
SS-RPN++     &0.861&0.653 & 0.755 &0.552 &0.543&0.464&0.606&0.656&0.734 & 0.448&0.455&0.542\\    
Su-RPN++     &0.881&0.665 & 0.776&0.592 &0.570&0.487& 0.640 &0.677 & 0.764 &0.471&0.466&0.560 \\ 
% SS-Su-RPN++ &0.905&0.685 &0.811&0.606 &0.629&0.530 &0.646&0.691&0.774 &0.499&0.499&0.596\\
%RPN++(reported)&0.914&0.696 &0.807&0.613 &-&- &0.694&0.733&0.800 &0.488&0.495&0.569\\
    \bottomrule
    \end{tabular}} 
\end{table*}




